TAXI: Evaluating Categorical Knowledge Editing for Language Models

Humans rarely learn one fact in isolation. Instead, learning a new fact induces knowledge of other facts about the world. For example, in learning a korat is a type of cat, you also infer it is a mammal and has claws, ensuring your model of the world is consistent. Knowledge editing aims to inject new facts into language models to improve their factuality, but current benchmarks fail to evaluate consistency, which is critical to ensure efficient, accurate, and generalizable edits. We manually create TAXI, a new benchmark dataset specifically created to evaluate consistency in categorical knowledge edits. TAXI contains 11,120 multiple-choice queries for 976 edits spanning 41 categories (e.g., Dogs), 164 subjects (e.g., Labrador), and 183 properties (e.g., is a mammal). We then use TAXI to evaluate popular editors' categorical consistency, measuring how often editing a subject's category appropriately edits its properties. We find that 1) the editors achieve marginal, yet non-random consistency, 2) their consistency far underperforms human baselines, and 3) consistency is more achievable when editing atypical subjects Our code and data are available at https://github.com/derekpowell/taxi.

==> tables/main_results2.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{2.5pt}     % slight adjustment to fit text width
\setlength{\cmidrulekern}{0.25em}
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccccc}
\toprule
 &  & Forward &  &  & Reversed & \\
% \toprule
 % & \multicolumn{4}{c}{\textbf{zsRE} (T5; F1 $\uparrow$)} & \multicolumn{4}{c}{\textbf{SCOTUS} (BERT; Acc $\uparrow$)}  & \multicolumn{5}{c}{\textbf{Hallucination} (GPT2-XL; PPL $\downarrow$)} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}%\cmidrule(lr){6-9} %\cmidrule(lr){10-14}
 & \textbf{FT} & \textbf{ROME} & \textbf{ICE} & \textbf{FT} & \textbf{ROME} & \textbf{IKE}\\

\midrule
\textbf{Edit Success} & .98 & .78 & 1.0 & .05 & .10 & 1.0\\
\midrule
\textbf{Consistency} & .31 & .48 & .55 & .05 & .12 & 1.0\\
% \midrule
\hspace{4mm}Shared Property & .73 & .76 & .91 & .10 & .21 & 1.0\\
\hspace{4mm}Modified Property & .23 & .43 & .47 & .04 & .10 & 1.0\\
% \midrule
\hfill Typical & .22 & .40 & .47 & .05 & .09 & 1.0\\
\hfill Atypical & .25 & .45 & .48 & .03 & .10 & 1.0\\
\bottomrule
\end{tabular}
}
\caption{Forward query performance for Finetuning (FT), ROME, and in-context (IKE) editing approaches on the \textsc{taxi} dataset. \textit{Consistency} indicates overall consistency across all property queries. \textit{Specificity} indicates consistency for unchanged properties, whereas \textit{generalization} indicates consitency for changed properties, which is reported for typical and atypical category exemplars.}\label{tab:main_results}
\end{table}

==> tables/per_category.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{3.7pt}     % slight adjustment to fit text width
\setlength{\cmidrulekern}{0.25em}
% \resizebox{\linewidth}{!}{
\begin{tabular}{lccc}
\toprule
 & \textbf{Finetune} & \textbf{ROME} & \textbf{ICE}\\
\midrule
Dog & 0 & 0 & 0\\
Cat & 0 & 0 & 0\\
Cow & 0 & 0 & 0\\
Bird & 0 & 0 & 0\\
Bee & 0 & 0 & 0\\
Fish & 0 & 0 & 0\\
Snake & 0 & 0 & 0\\
\midrule
Avg & 0 & 0 & 0\\
\bottomrule
\end{tabular}
% }
\caption{Per-Category Results.}\label{tab:entity_results}
\end{table}


==> tables/taxonomy_full.tex <==
\begin{table*}[t]
\centering
\setlength{\tabcolsep}{3.7pt}     % slight adjustment to fit text width
\setlength{\cmidrulekern}{0.25em}
% \resizebox{\linewidth}{!}{
\begin{tabular}{cp{.25\linewidth}p{.6\linewidth}}
\toprule
 & \textbf{Exemplars} & \textbf{Properties} \\
\midrule
Animals &  & \\
 \midule
Dog & Labrador, Chihuahua, Pekingese, Bichon Frise & Born in a litter, has fur, is domesticated, has four legs, kept as pets, likes to fetch, barks, walks, baby is a puppy, is a mammal \\
\midrule
Cat & Siamese, Persian, Abyssinian, Chartreux & Born in a litter, has claws, has fur, is domesticated, has four legs, kept as pets, likes to chase, meows, walks, baby is a kitten, eats meat \\
\midrule
Cow & Holstein, Jersey, Galloway, Hereford & Is a mammal, born alone, has hooves, has fur, is domesticated, has four legs, kept for their milk, likes to graze, moos, walks, baby is a calf, eats grain, makes milk \\
\midrule
Bird & sparrow, canary, woodpecker, Partridge & Is an aves, hatched from egg, has wings, has feathers, chirps, flies, baby is a chick, can fly, is wild\\
\midrule
Bee & Bumblebee, Honeybee, Megachile, Apis Mellifera  & Is an insect, has wings, has six legs, buzzes, flies, makes honey, can fly \\
\midrule
Fish & Trout, salmon, Flounder, tilapia & Hatched from an egg, has scales, has fins, has no legs, caught and eaten, swims, lives in water, can swim, is wild \\
\midrule
Snake & Cobra, python, copperhead, Gaboon viper & Hatched from an egg, has scales, no legs, people avoid, hisses, slithers, is wild \\
\bottomrule
\end{tabular}
% }
\caption{Taxonomic details for superordinate category "animals" from the \textsc{taxi} benchmark dataset. The first two listed exemplars are typical exemplars. }\label{tab:taxonomy}
\end{table*}
